Continual Novelty Detection

Novelty Detection methods identify samples that are not representative of a model's training set thereby flagging misleading predictions and bringing a greater flexibility and transparency at deployment time. However, research in this area has only considered Novelty Detection in the offline setting. Recently, there has been a growing realization in the computer vision community that applications demand a more flexible framework - Continual Learning - where new batches of data representing new domains, new classes or new tasks become available at different points in time. In this setting, Novelty Detection becomes more important, interesting and challenging. This work identifies the crucial link between the two problems and investigates the Novelty Detection problem under the Continual Learning setting. We formulate the Continual Novelty Detection problem and present a benchmark, where we compare several Novelty Detection methods under different Continual Learning settings. We show that Continual Learning affects the behaviour of novelty detection algorithms, while novelty detection can pinpoint insights in the behaviour of a continual learner. We further propose baselines and discuss possible research directions. We believe that the coupling of the two problems is a promising direction to bring vision models into practice.

==> latex/BaselineTab.tex <==
\resizebox{\columnwidth}{!}{
\small
\begin{tabular}{ c|c|c|c|c|c|c|c|c  }
 %\hline
%Setting & Method &mean  previous tasks AUC &mean current AUC & mean combined AUC& mean AUC& mean combined deterr&mean Forg \vs \IN &\F \vs \Out\\ \hline
Setting & Method & m.P.AUC $\uparrow$ &m.R.AUC$\uparrow$  & mC.AUC$\uparrow$ & mAUC$\uparrow$ &m.DER$\downarrow$ &F/IN$\downarrow$ &F/Out$\downarrow$\\ \hline
\multirow{3}{4em}{Multi-head\\\fine} &\nav& 66.1 & 81.6 & 74.1 & 71.0 & 31.7 & 31.0 & 43.8  \\ 
&\Ba& 67.7 & 83.0 & 75.3 & 72.5 & 30.7 & 30.8 & 43.6  \\
%&\Bb & 60.2 & 82.8 & 75.5 & 72.5 & 30.6 & 30.2 & 43.8 \\
& \Bb  & 68.1 & 83.2 & 75.8 & 72.8 & 30.4 & 30.2 & 43.8   \\  
\hline
\multirow{2}{4em}{Multi-head\\MAS} &  \nav& 78.1 & 76.7 & 76.5 & 78.2 & 29.7 & 14.5 & 43.4  \\
&\Ba  & 78.4 & 77.1 & 74.1 & 78.5 & 31.7 & 22.8 & 40.8   \\
%&\Bb & 70.0 & 77.5 & 75.7 & 78.9 & 30.6 & 19.1 & 41.9   \\ 
&\Bb & 79.1 & 77.7 & 75.8 & 79.2 & 30.5 & 20.6 & 41.9\\
\hline
\multirow{2}{4em}{Multi-head\\LWF}
 &\nav  & 79.7 & 80.5 & 76.9 & 80.3 & 29.5 & 17.1 & 42.9   \\
 &\Ba  & 80.3 & 82.2 & 75.8 & 81.1 & 29.2 & 22.6 & 39.8       \\
 %&\Bb & 71.6 & 82.2 & 77.9 & 81.3 & 28.2 & 18.6 & 41.4   \\ 
 &\Bb  & 80.8 & 82.4 & 78.0 & 81.6 & 28.2 & 20.4 & 41.0 \\
 \hline
 \multirow{2}{4em}{Shared-head\\ER-10s}
 &\nav & 76.2 & 71.1 & - & 75.0 & 31.0 & 25.6 & 42.5      \\
 &\Ba  & 75.9 & 71.2 & - & 74.8 & 30.8 & 28.0 & 41.1  \\
 %&\Bb & 68.0 & 71.7 & - & 75.2 & 30.7 & 26.1 & 41.7  \\ 
 &\Bb & 77.1 & 72.5 & - & 76.0 & 30.0 & 26.2 & 41.5    \\
 \hline
   \multirow{2}{4em}{Shared-head\\ER-25s}
  & \nav & 78.4 & 70.5 &- & 76.6 & 29.8 & 22.8 & 42.2  \\ 
 & \Ba  & 78.7 & 69.7 & -& 76.4 & 29.4 & 25.5 & 41.0 \\
% &\Bb & 70.4 & 70.5 & - & 77.0 & 29.2 & 23.4 & 41.5  \\
 &\Bb&  79.8 & 71.4 & - & 77.7 & 28.6 & 23.7 & 41.4  \\
 \hline
  \multirow{2}{4em}{Shared-head\\ER-50s}
  &\nav & 80.1 & 69.8 & - & 77.8 & 28.4 & 22.2 & 41.0   \\
  &\Ba & 79.1 & 66.1 & - & 76.1 & 29.2 & 25.9 & 39.2 \\
 %& \Bb & 71.2 & 67.9 & - & 77.3 & 28.5 & 23.0 & 40.6  \\
  &\Bb  & 80.7 & 68.9 & - & 78.0 & 27.8 & 23.5 & 40.1     \\ %\hline
 \end{tabular}}

==> sections/old_intro.tex <==
Continual learning has gained increased interest in the past years for its applicability %\daniel{The message here is that, in practice, many settings are subject to continual learning, but this fact is usually ignored.} 
to real life scenarios. It provides computer vision models with the ability to update and expand their acquired knowledge across time with minimal computation and memory overhead. %\daniel{This setting, when model [...] is also referred to as lifelong learning or incremental learning.}
The setting when a model is trained incrementally on a new set of classes or new tasks is referred to as lifelong learning, incremental learning or \textit{continual learning}.
Continual learning is inspired by the human ability to continuously acquire new knowledge and adapt to new scenarios. However, humans and mammals in general are known with their distinctive ability to discriminate familiar objects from novel objects~\cite{antunes2012novel,broadbent2010object}. When faced with a novel object, humans try to discover and acquire information on the novel object and thus adding it to the set of familiar known objects. While the later is what continual learning describes, the former is what novelty detection methods aims at achieving. %    ability update its acquired knowledge and skills and constantly expand it 
% yet it assumes no direct connection between the new training episodes and what is seen at deployment time. Humans usually ask for information on things that they don't know which will later become covered by their knowledge.

\textit{Novelty} or Out of Distribution or Anomaly \textit{Detection} methods deal with the problem of detecting input data that do not belong to the task that a given model has been trained for~\cite{hendrycks2016baseline}. This can be especially useful at deployment time in order to avoid  misleading predictions on samples that are irrelevant to the concerned task. This also relates to providing the model with a  ``no'' option, when an input is out of its knowledge scope, enhancing the safety conditions. \\
Yet continual learning and novelty detection are currently studied as independent problems. 
{Let us consider the setting of learning a sequence of tasks from the same domain.} 
Imagine for example an object detection or recognition model operating on input from driving scenes. For simplicity, let us say that the model is initially trained on recognizing cars and pedestrians given available annotations. %after after Objects that have been annotated given gathered data and a certain annotation budget. 
At deployment time, new objects are spotted \eg, cyclists or e-scooter. Ideally, those novel objects can be later annotated after which the model will be trained expanding its current knowledge to contain car, pedestrian, cyclist and e-scooter. This process can continue as long as new objects of interest are being detected and later annotated.  While such scenario is very relevant to real life applications, it is very different from the setting under which existing novelty detection or continual learning methods are operating. \\
% If the input data detected as novel are of interest for the model task, they should be later annotated and added to the training set.
% \daniel{The purpose of this paragraph is not clear. Seems disconnected from the previous paragraph (it's not but bear with me). The story is this: in previous paragraph we illustrate an example of adding new categories from the same domain. In this one we say that most methods deal with new tasks from different domains.}
Most  novelty detection methods are designed and tested for detecting input data drawn from datasets other than those used for training (\eg, training on CIFAR10 and detecting SVHN images~[refs]) in which the discrepancy between the datasets can be exploited
%by the novelty detection method as more of  a shift in the input domain,
rather than a difference in the represented objects.  
%\daniel{( datasets/domains/task is a bit confusing)}
% In practice novel objects  is likely to correspond  , when models are deployed in a real test environment,
% It has been noted that when novel objects are from different categories of the same domain, detection of them is harder~\cite{liang2017enhancing}.
It has been noted that novel objects detection is harder when they are from different categories of the same domain~\cite{liang2017enhancing}.
%\daniel{At this point, there is break in the flow of the story, I think.}
As mentioned earlier, the detected relevant novel  objects, can be annotated and trained on, resulting in an expansion in the knowledge covered by the trained model.
% As continual learning when constrained to a limited computational budget suffers from forgetting, it is intriguing to discover how the forgotten data are then treated.
% \nikolay{Being constrained to a limited computational budget, continual learning suffers from forgetting, which opens a question about how the forgotten data are then treated.} \daniel{$\leftarrow$ This is mentioned in Related Work. Maybe here is not the best place to put it :(, but let's see if we address the concern later.}

In fact, the knowledge covered by the continually trained model is not only expanding but shifting over time. \\
% \daniel{At this point we need closure. We say that a common situation is this, but most methods deal with that. Shall we say here that we study both situations?}
%As we mentioned, if novel detected objects are of interest for the current application, %human annotators will provide the system with the previously unknown labels and the %model has to be trained on these newly detected objects. 
%The training distribution is expected to grow and new classes will be asked to be trained on new completely new tasks.
In this work, we propose and formulate the problem of Continual Novelty Detection, a problem that arises when novelty detection methods are applied in a continual learning scenario in which the concerned prediction model is continuously updating its existing knowledge. 
%Continual learning has become a very hot research topic nowadays due to its relevance to many real life applications. %ADD EXAMPLES.
%To do, add somwhere analogy to humans ability to tell at any point if a given input is faimilar or not,
%   \begin{figure}[t!]
% \centering
% \includegraphics[width=0.35\textwidth]{latex/Figures/idea.png}
%   \caption{Ideal system condition, the system transitions between learning and prediction. While given prediction, the model has to detect novel objects. Once novel objects are gathered a new learning step can be carried on. }
%   \label{fig:examples}
%   \end{figure}
\begin{figure}[t]
\centering
\includegraphics[width=0.4\textwidth]{latex/Figures/in_out_ill.png}  \caption{Illustration of three different sets of samples constructed in the context of continual learning. %\daniel{In S2, samples move with regard to their positions in S1. Do we mean to imply the change in representation because of the newly learned task 2? Or should they remain in place, and we just change the boundaries?}
}
  \label{fig:expanded seen set}
  \vspace*{-0.6cm}
  \end{figure}
% The main obstacle of continual learning is the catastrophic forgetting of previous knowledge when new information is learned. This is usually due the limited or no access to previously learned data. 
% While many solutions have been proposed to overcome the catastrophic forgetting phenomenon and allow the incremental learning of new classes or new tasks (see~\cite{de2019continual} for a survey), these methods assume that the new classes arrive in batches along with their labelled data while at test time these methods are deployed in the same setting as standard supervised learning methods where prediction have to be made on test samples that are assumed to belong to the learned classes or tasks.  
% Very recently, new methods were proposed to detect task boundaries, \ie, when a new task is encountered that is different from the existing training data. However, this kind of detection, \nikolay{also?} assumes that samples of new tasks are received in batches along with their labels and mostly rely on the statistics of the loss function for such detection~[add Ref].
% An important missing gap for these continual learning methods to be deployed in practice is the ability of detecting novel input that do not belong to any of the previously learned experiences.  Once novel input is detected, a request for annotation can be generated and then a new phase of learning could take place.  
% More concretely, we  investigate whether  the sequential learning nature affects the novelty detection behaviour, and whether a need emerges for methods  that are aware of the model continuously updated knowledge.
% One could ask how current existing novelty detection method perform when deployed in such a continual learning scenario. In another word, does the sequential learning nature affects the detection ability of such methods, do we need to develop new methods that can be aware of the model expanded knowledge and hence their detection of novel objects is updated consequently. 
To this end, we formulate the continual novelty detection problem and divide the set of inspected samples into three subsets of (\IN) samples covering those of previously and recently learned concepts, {\tt Forgotten} samples subject to mistaken predictions as a result of continual learning and, finally, the (\Out) samples, covering those of yet unseen concepts. 
\textcolor{red}{With the goal of understanding existing novelty detection behaviour in this setting and whether novelty detection methods are capable of coping with a dynamic (\IN) set and further how possibly forgotten samples are treated by novelty detection methods, we construct a benchmark on which we evaluate several existing novelty detection methods.} \textcolor{red}{We note a clear connection between continual learning and novelty detection and insights that novelty detection methods can tell about a continual learner behaviour and vise versa.} We also highlight the need for developing new novelty detection methods that are closely linked to the trained model and the deployed continual learning method.\\ 
To stimulate research on this problem, we further propose additional simple and cheap  baselines that improve  over existing methods and highlight possible promising directions.
Our contributions are as follows:
1)~we are the first to investigate the novelty detection problem under the continual learning setting;
2)~we establish  benchmarks for the described continual novelty detection problem and compare different existing methods;
3)~we discuss possible directions to tackle this problem and propose new baselines improving over existing methods.
% Knowledge is always expanded/updated, previously out-of-distribution samples become in-distribution. How to model a growing and a changing distribution
